KnowGraph: Knowledge-Enabled Anomaly Detection via Logical Reasoning on Graph Data

Graph-based anomaly detection is pivotal in diverse security applications, such as fraud detection in transaction networks and intrusion detection for network traffic. Standard approaches, including Graph Neural Networks (GNNs), often struggle to generalize across shifting data distributions. Meanwhile, real-world domain knowledge is more stable and a common existing component of real-world detection strategies. To explicitly integrate such knowledge into data-driven models such as GCNs, we propose KnowGraph, which integrates domain knowledge with data-driven learning for enhanced graph-based anomaly detection. KnowGraph comprises two principal components: (1) a statistical learning component that utilizes a main model for the overarching detection task, augmented by multiple specialized knowledge models that predict domain-specific semantic entities; (2) a reasoning component that employs probabilistic graphical models to execute logical inferences based on model outputs, encoding domain knowledge through weighted first-order logic formulas. Extensive experiments on these large-scale real-world datasets show that KnowGraph consistently outperforms state-of-the-art baselines in both transductive and inductive settings, achieving substantial gains in average precision when generalizing to completely unseen test graphs. Further ablation studies demonstrate the effectiveness of the proposed reasoning component in improving detection performance, especially under extreme class imbalance. These results highlight the potential of integrating domain knowledge into data-driven models for high-stakes, graph-based security applications.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> misc.tex <==
% To reduce the computational complexity of training the MLN, we follow \cite{zhang2022care} and employ variational inference, aiming to optimize the variational evidence lower bound (ELBO) of the data log-likelihood. This is due to the intractability of directing optimizing \ref{eq:joint_p} since it requires direct computation of $Z(w)$ and integration over all observed predicates $\mathcal{O}$ and unobserved predicates $\mathcal{U}$. The ELBO is formulated as follows:
% \begin{equation}
% \begin{split}
% \log P_{w}(\mathcal{O}) \ge \mathcal{L}_{\mathrm{ELBO}}(Q_{\theta}, P_{w}) &=  \mathbb{E}_{Q_{\theta}(\mathcal{U} | \mathcal{O})}\left[\log P_{w}(\mathcal{O}, \mathcal{U})\right] \\
% & - \mathbb{E}_{Q_{\theta}(\mathcal{U} | \mathcal{O})}\left[\log Q_{\theta}(\mathcal{U} | \mathcal{O})\right],
% \end{split}
% \end{equation}

% where $Q_{\theta}(\mathcal{U}|\mathcal{O})$ represents the variational posterior distribution. The representation of sensor outputs and knowledge rules as a graph motivates the use of GCNs for encoding $Q_\theta(\cdot)$. 

% To determine the weights of the MLN, $w$, we adopt a variational EM algorithm to refine the ELBO. Given the absence of input $x$, all variables like $\texttt{IsNTLM}(x)$ can be treated as unobserved variables, setting $\mathcal{O}$ as an empty set and focusing our optimization on sensor outputs $\pT={t_1, t_2, ...,t_L }$. The resulting optimization goal is to minimize the negative KL divergence between the variational distribution $Q_{\theta}(\pT)$ and the actual distribution $P_w(\pT)$, effectively approximating $P_w(\pT)$ through $Q_{\theta}(\pT)$. The following simplified equation captures this process:
% \begin{equation}
%     \label{eq:new-elbo}
%     \begin{split}
%     \mathcal{L}_{\mathrm{ELBO}}(Q_{\theta}, P_{w}) := \mathbb{E}_{Q_{\theta}(\pT)}[\log P_{w}(\pT)] & - & \mathbb{E}_{Q_{\theta}(\pT)}[\log Q_{\theta}(\pT)].
%     \end{split}
% \end{equation}
% This streamlined approach enables the efficient approximation of the desired distribution through the MLN training process, composed of two steps. 

% \paragraph{E-step}
% During the E-step, the MLN weights $w$ for the knowledge rules are constant and the GCN parameters $Q_{\theta}$ are updated to reduce the KL divergence between $Q_{\theta}(\pT)$ and $P_w(\pT)$. Following CARE \cite{zhang2022care} we approximate $P_w(\pT)$ with a mean-field distribution and express the joint distribution of outputs of sensors in the following:
% \begin{equation}
% \label{eq:mean-field}
%    Q_{\theta}(\pT):= \prod\nolimits_{t_i \in \pT} Q_{\theta}(t_i),
% \vspace{-2mm}
% \end{equation}
% where the sum of the $Q_{\theta}(t_i)$ is constrained to 1. We approximate $Q_{\theta}$ with a GCN, where $\theta$ represents the GCN's parameters. Each node is the output prediction of a sensor whose value represents the confidence of the corresponding class. Additionally, we train a class embedding vector $\vec{\mu_i}$ for each node to avoid relying on scaler values. The input for each node is then the product of the class prediction confidence $z_i$ and its respective class embedding vector $\vec{\mu_i}$, enhancing the model's expressiveness. 

% Based on the mean-field approximation the ELBO from Eq.~\ref{eq:new-elbo} can thus be rewritten as:
% \begin{small}
% \begin{equation}
% \begin{aligned}
% \label{eq:reelbo}
% \mathcal{L}_{\mathrm{ELBO}}\left(Q_{\theta}, P_{w}\right) = \mathbb{E}_{Q_{\theta}(\mathcal{P})} & \left(  \sum_{f \in \mathcal{F}} w_ff(t_1,...,t_L) - \log Z(w) \right) \\
% &- \mathbb{E}_{Q_{\theta}(\pT)}\log Q_{\theta}(\pT),
% \end{aligned}
% \end{equation}
% \end{small}
% where $\log Z(w)$ here is a constant since the MLN weights are fixed during the E-step. Since the gradients of the GCN cannot be directly backpropagated, we use the explicit form of the gradient derived in \cite{zhang2022care}:
% \begin{equation}
% \label{eq:gcn-gradient}
% \mathbb{E}_{Q_{\theta}(\pT)}\left(\sum_{f \in \mathcal{F}} w_ff(t_1,...,t_L) -\log Q_{\theta}(\pT)\right)\nabla_\theta\log Q_{\theta}(\pT).
% \end{equation}

% Since we consider learning tasks where label information is available for each input during training, we follow \cite{zhang2022care} and use a supervised negative log-likelihood term to improve optimization:
% \begin{equation}
% \mathcal{L}_{\text{supervised}}(Q_{\theta})= -\sum_{i=1}^L \log Q_{\theta}\left( \text{GroundTruth}(t_i)\right),
% \end{equation}
% where $\text{GroundTruth}(t_i)$ denotes the actual label associated with predicate $t_i$ during training. Therefore, the enhanced E-step optimization objective becomes:
% \begin{equation}
% \label{eq:final}
% \mathcal{L}_{\text{new}}(Q_{\theta}) =\mathcal{L}_{\text{ELBO}}(Q_{\theta}, P_{w})-\eta\mathcal{L}_{\text{supervised}}(Q_{\theta}),
% \end{equation}
% with $\eta$ serving as a hyperparameter to balance the importance of the ELBO term against the supervised learning term. This approach ensures that the embeddings $\vec{\mu}$ are refined during the optimization of the GCN, leveraging the chain rule to augment model expressiveness.

% During inference, class predictions are made based on the marginal probabilities $Q_{\theta}(t_i)$, effectively acting as a knowledge-informed adjustment to initial predictions.

% \paragraph{M-step}
% Conversely, the M-step involves fixing $Q_{\theta}$ while updating the weights $w$ to optimize the log-likelihood function $\mathbb{E}_{Q_{\theta}(\pT) }\left[\log P_{w}( \pT)\right]$. This aims to maximize the term 
% \begin{equation}
% \label{eq:loglikelihood}
% \mathbb{E}_{Q_{\theta}(\mathcal{T})} \log \frac{\exp\{\sum_{f \in \mathcal{F}} w_f f(t_1,...,t_L)\}}{\sum_{t'_1,...t'_L} \exp\{\sum_{f \in \mathcal{F}} w_ff(t_1',...,t_L')\}}.
% \end{equation}
% Since directly integrating over all variables is intractable, we follow \cite{zhang2022care} and optimize the pseudo-likelihood~\cite{Besag1977EfficiencyOP} instead, which is formulated as:
% \begin{equation}
% \begin{aligned}
% P_{w}^*(t_1,..., t_L) := \prod_{i=1}^{L} P_{w}\left(t_{i} | MB\left(t_{i}\right)\right), 
% \end{aligned}
% \end{equation}
% where $f\left(t_{i}=0\right)$ and $f\left(t_{i}=1\right)$ reflect the formula $f$'s ground truth values under the hypothetical scenarios of $t_i$ being 0 or 1, respectively, with other variables held constant.

% The strategy to address the original complex log-likelihood involves maximizing the expectation of the pseudo-log-likelihood, $\mathbb{E}_{Q{\theta}(\mathcal{T})}\left[\log P_w^*\left(\mathcal{T}\right)\right]$. This maximization is facilitated through the estimation of the gradient concerning the formula weight $w$ via multiple samplings from the variational distribution $Q_{\theta}$.

%     \item \textbf{E-step:} Keeping MLN weights constant, we optimize the GCN parameters $Q_{\theta}$ to reduce the KL divergence between $Q_{\theta}(\pT)$ and $P_w(\pT)$. This involves a mean-field approximation to handle the scale, assuming variable independence and optimizing the sensor outputs' joint distribution. The adapted ELBO for our scenario is expressed as:
%     \item \textbf{M-step:} With fixed GCN parameters, the MLN weights $w$ are updated to enhance the expected log-likelihood. Due to the infeasibility of calculating the partition function, we approximate it with a pseudo-likelihood, thereby maximizing its expectation:
%     \begin{equation}
%     \mathbb{E}_{Q_{\theta}(\mathcal{T})}\left[\log P_w^*\left(\mathcal{T}\right)\right],
%     \end{equation}
%     where the optimization employs sampling from the variational distribution $Q_{\theta}$.
% \end{itemize}


==> tables/ebay_calibration.tex <==
\begin{table}
  \centering
  \caption{Overall performance of baselines and the sensing-reasoning framework. We observe greater performance on both transductive and inductive settings. We report AUC and average precision with $k=0.5$}
    \begin{tabular}{l|cccc}
    \toprule
    Sensor & Transductive & Inductive \\
    \midrule
    GCN {\scriptsize~\cite{kipf2017semisupervised}} & 0.723 & 0.0001 \\
    DGI {\scriptsize~\cite{veličković2018deep}} & 0.587 & 0.0001 \\
    Reasoning (Ours) & \textbf{0.755} & \textbf{0.121} \\
    + Weight Ensemble & \textbf{0.731} & \textbf{0.167} \\
    \bottomrule
    \end{tabular}
  \label{tab:overall}
\end{table}




==> tables/ebay_fpr.tex <==
\begin{table}[ht]
\centering
\caption{True positive (TP) rates of DGI \cite{veličković2018deep} baseline and \name~ at  different false positive (FP) rates. \name~ achieves higher TP rates, especially at higer FP rates. \bo{bold. can we evaluate more and is this final? use the same format, why one \% one 0.xxx}}
\begin{tabular}{lcc}
\toprule
Method & FP & TP \\
\midrule
\multirow{3}{*}{DGI} & 0.5 & 0.0 \\
                     & 1.0 & 0.0096 \\
                     & 2.0 & 0.0096 \\
\midrule
\multirow{3}{*}{\textbf{\name}} & 0.5 & 0.0 \\
                                          & 1.0 & 0.0096 \\
                                          & 2.0 & 0.0144 \\
\bottomrule
\end{tabular}
\label{tab:overall}
\end{table}


==> tables/ebay_inductive.tex <==
\begin{table*}[!t]
\centering
\caption{Performance Metrics Over Different Days}
\label{tab:performance-days}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Methods & 0 days & 1 day & 2 days & 3 days & 4 days & 20 days \\
\midrule
Baseline & 0.8924/0.5868 & 0.4920/0.0001 & 0.499/0.0001 & 0.5049/0.0001 & 0.4890/0.0001 & 0.498/0.0001 \\
Price/Shipping Rule & 0.531/0.0578 & 0.5426/0.0800 & 0.5191/0.0230 & 0.5335/0.0627 & 0.5250/0.0501 & 0.5513/0.0992 \\
Sensing-reasoning & 0.978/0.7545 & 0.587/0.1195 & 0.564/0.0358 & 0.596/0.0789 & 0.558/0.0668 & 0.609/0.1211 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/ebay_overall_old.tex <==
\begin{table}
  \centering
  \caption{Overall performance of baselines and the sensing-reasoning framework. We observe greater performance on both transductive and inductive settings. We report AUC and average precision with $k=0.5$}
    \begin{tabular}{l|cccc}
    \toprule
    Sensor & Transductive & Inductive \\
    \midrule
    GCN {\scriptsize~\cite{kipf2017semisupervised}} & 0.723 & 0.0001 \\
    DGI {\scriptsize~\cite{veličković2018deep}} & 0.587 & 0.0001 \\
    \textbf{GraphLR (Ours)} & \textbf{0.755} & \textbf{0.121} \\
    \textbf{+ PCS} & \textbf{0.731} & \textbf{0.167} \\
    \bottomrule
    \end{tabular}
  \label{tab:overall}
\end{table}



